SPROUT: Predicting Objective-Grounded Prompt Utility for Efficient Text-to-Image Preference Tuning

Preference tuning of text-to-image diffusion models spends most of its compute generating candidate images, yet training prompts are typically sampled uniformly at random, wasting compute generating images that provide too little signal for model alignment. To best utilize the available compute, we study prompt selection, where at each iteration we identify the most useful prompts for preference tuning. We separate prompt selection into a utility score, an estimator of that utility score, and batch selection. Within this framework, we propose Selection by PRedicting Objective-grounded UTility (SPROUT). The utility score is predicted on every prompt in the pool, including unseen prompts, by a text-only model, refit after every iteration on all utilities observed so far. A randomized acceptance rule then turns these predictions into a batch, so no images are generated beyond those used for training. For direct group preference optimization (DGPO), the objective-grounded utility is the norm of the gradient that the objective produces from a prompt's group of images. Fine-tuning Stable Diffusion 1.5 with DGPO on GenEval, SPROUT matches the final score of uniform sampling in about 44% of the iterations and improves the area under the learning curve with respect to both uniform sampling and CGPO, a recent variance-based prompt sampler. The efficiency gains hold under four held-out reward models never used in training, and the ranking of methods carries over to DPG-Bench and T2I-CompBench++. Our code is available at https://github.com/ADDAPT-ML/SPROUT.

==> tab/batch16_judges.tex <==
\begin{tabular}{lcccc}
\toprule
Method & PickScore & HPS v2.1 & Aesthetic & ImageReward \\
\midrule
CGPO~\cite{Li_2026_CVPR} & +0.4\,[-3.5, +4.3] & -0.8\,[-6.8, +5.1] & +1.4\,[-5.1, +7.9] & -3.7\,[-16.0, +8.5] \\
SPROUT w/ variance & \textbf{+4.0\,[+0.2, +7.7]} & +3.7\,[-0.3, +7.7] & +3.7\,[-2.1, +9.5] & \textbf{+6.3\,[+2.9, +9.6]} \\
SPROUT & +3.4\,[-3.0, +9.7] & +2.3\,[-0.9, +5.5] & +3.6\,[-0.9, +8.1] & +3.3\,[-3.7, +10.3] \\
\bottomrule
\end{tabular}


==> tab/pickscore.tex <==
\begin{tabular}{lccccc}
\toprule
 & & \multicolumn{4}{c}{$\Delta$nAULC vs Uniform} \\
Method & PickScore@100 & PickScore & HPS v2.1 & Aesthetic & ImageReward \\
\midrule
Base model & 19.971 & -- & -- & -- & -- \\
Uniform & 20.355\,$\pm$\,0.033 & -- & -- & -- & -- \\
Ours (variance) & 20.365\,$\pm$\,0.042 & +0.1\,[-5.5, +5.8] & -0.4\,[-1.6, +0.7] & -0.4\,[-4.2, +3.3] & +0.2\,[-5.7, +6.1] \\
Ours (update norm) & 20.351\,$\pm$\,0.021 & -1.5\,[-4.4, +1.4] & -1.0\,[-4.8, +2.9] & -0.7\,[-3.2, +1.9] & -1.0\,[-5.8, +3.8] \\
\bottomrule
\end{tabular}

